Axiomatizing the Logic of Ordinary Discourse

Most non-classical logics are subclassical, that is, every inference/theorem they validate is also valid classically. A notable exception is the three-valued propositional Logic of Ordinary Discourse (OL) proposed and extensively motivated by W. S. Cooper as a more adequate candidate for formalizing everyday reasoning (in English). OL challenges classical logic not only by rejecting some theses, but also by accepting non-classically valid principles, such as so-called Aristotle's and Boethius' theses. Formally, OL shows a number of unusual features - it is non-structural, connexive, paraconsistent and contradictory - making it all the more interesting for the mathematical logician. We present our recent findings on OL and its structural companion (that we call sOL). We introduce Hilbert-style multiple-conclusion calculi for OL and sOL that are both modular and analytic, and easily allow us to obtain single-conclusion axiomatizations. We prove that sOL is algebraizable and single out its equivalent semantics, which turns out to be a discriminator variety generated by a three-element algebra. Having observed that sOL can express the connectives of other three-valued logics, we prove that it is definitionally equivalent to an expansion of the three-valued logic J3 of D'Ottaviano and da Costa, itself an axiomatic extension of paraconsistent Nelson logic.

==> macros.tex <==
\makeatletter
\newcommand{\dotfrac}[2]{
\mathchoice
{\ooalign{$\genfrac{}{}{0pt}{0}{#1}{#2}$\cr\leavevmode\cleaders\hb@xt@ .22em{\hss $\displaystyle\cdot$\hss}\hfill\kern\z@\cr}}
{\ooalign{$\genfrac{}{}{0pt}{1}{#1}{#2}$\cr\leavevmode\cleaders\hb@xt@ .22em{\hss $\textstyle\cdot$\hss}\hfill\kern\z@\cr}}
{\ooalign{$\genfrac{}{}{0pt}{2}{#1}{#2}$\cr\leavevmode\cleaders\hb@xt@ .22em{\hss $\scriptstyle\cdot$\hss}\hfill\kern\z@\cr}}
{\ooalign{$\genfrac{}{}{0pt}{3}{#1}{#2}$\cr\leavevmode\cleaders\hb@xt@ .22em{\hss $\scriptscriptstyle\cdot$\hss}\hfill\kern\z@\cr}}
}
\makeatother

%\makeatletter
%\newcommand\dotover{\leavevmode\cleaders\hb@xt@ .22em{\hss $\cdot$\hss}\hfill\kern\z@}
%\newcommand{\dotfrac}[2]{
%\ooalign{$\genfrac{}{}{0pt}{0}{#1}{#2}$\cr\dotover\cr}
%}
%\makeatother

\newcommand{\Fixed}[2]{{\color{blue} #2}\textsuperscript{\tiny\textbf{FIX{#1}}}}

\newcommand{\tuple}[1]{{\langle #1\rangle}}
\newcommand{\conn}{\copyright}
\newcommand{\sub}{\mathsf{sub}}
\newcommand{\var}{\mathsf{var}}


\newcommand{\mcCooOL}{\mathrm{OL}^{\SetSetCR{}}}
\newcommand{\CooOL}{\mathrm{OL}}
\newcommand{\SOL}{\mathrm{sOL}}
\newcommand{\mcSOL}{\mathrm{sOL}^{\SetSetCR{}}}

\newcommand{\lordimpneg}{\curlyvee}
\newcommand{\dtimpneg}{\Rightarrow_{\star}}

% Names of the logics
\newcommand{\OL}{\textbf{\textup{O}}}
\newcommand{\LThreeName}{\textbf{\textup{\L$_3$}}}
\newcommand{\LPName}{\textbf{\textup{LP}}}
\newcommand{\LPImpName}{\textbf{\textup{LP}$^\ararr{}$}}
\newcommand{\BKName}{\textbf{\textup{BK}}}
\newcommand{\PWKName}{\textbf{\textup{PK}}}
\newcommand{\JThreeName}{\textbf{\textup{J3}}}
\newcommand{\GThreeName}{\textbf{\textup{G3}}}
\newcommand{\SKName}{\textbf{\textup{K}}}
\newcommand{\SThreeName}{\textbf{\textup{S3}}}
\newcommand{\MSevenName}{\textbf{\textup{L7}}}
\newcommand{\MEightName}{\textbf{\textup{L8}}}
\newcommand{\SetteName}{\textbf{\textup{S}}}
\newcommand{\PostName}{\textbf{\textup{P3}}}
\newcommand{\BelnapDunnName}{\textbf{\textup{E}}}

\newcommand{\LName}{\mathbf{L}}



\newcommand{\lukConj}{\ensuremath{\land_{\mathsf{min}}}}
\newcommand{\lukDisj}{\ensuremath{\lor_{\mathsf{max}}}}
\newcommand{\lukImp}{\ensuremath{\to_{\textrm{\LThreeName}}}}
\newcommand{\lukNeg}{\ensuremath{\lnot_{\LThreeName}}}
\newcommand{\lukDiam}{\ensuremath{\Diamond_{\LThreeName}}}

\newcommand{\postNeg}{\ensuremath{\lnot_{\PostName}}}

\newcommand{\setteImp}{\ensuremath{\to_{\SetteName}}}
\newcommand{\setteNeg}{\ensuremath{\lnot_{\SetteName}}}

\newcommand{\KleeConj}{\ensuremath{\land_{\SKName}}}
\newcommand{\KleeDisj}{\ensuremath{\lor_{\SKName}}}
\newcommand{\KleeNeg}{\ensuremath{\lnot_{\SKName}}}
\newcommand{\KleeImp}{\ensuremath{\to_{\SKName}}}

\newcommand{\BKleeConj}{\ensuremath{\land_{\BKName}}}
\newcommand{\BKleeDisj}{\ensuremath{\lor_{\BKName}}}
\newcommand{\BKleeNeg}{\ensuremath{\lnot_{\BKName}}}
\newcommand{\BKleeImp}{\ensuremath{\to_{\BKName}}}

\newcommand{\WKleeConj}{\ensuremath{\land_{\PWKName}}}
\newcommand{\WKleeDisj}{\ensuremath{\lor_{\PWKName}}}
\newcommand{\WKleeNeg}{\ensuremath{\lnot_{\PWKName}}}
\newcommand{\WKleeImp}{\ensuremath{\to_{\PWKName}}}

\newcommand{\SobocConj}{\ensuremath{\land_{\SThreeName}}}
\newcommand{\SobocDisj}{\ensuremath{\lor_{\SThreeName}}}
\newcommand{\SobocNeg}{\ensuremath{\lnot_{\SThreeName}}}
\newcommand{\SobocImp}{\ensuremath{\to_{\SThreeName}}}

\newcommand{\LPImp}{\ensuremath{\to_{\LPName}}}

\newcommand{\JThreeImp}{\ensuremath{\to_{\JThreeName}}}
\newcommand{\LukPoss}{\ensuremath{\Diamond_{}}}

\newcommand{\HImp}{\ensuremath{\to_{\GThreeName}}}
\newcommand{\HNeg}{\ensuremath{\lnot_{\GThreeName}}}

\newcommand{\DSetOne}{\{\tv\}}
\newcommand{\DSetTwo}{\{\tv,\uv\}}

\newcommand{\EmptySet}{\varnothing}
\newcommand{\SetFmla}{{\upshape\textsc{Set-Fmla}}}
\newcommand{\SetSet}{{\upshape\textsc{Set-Set}}}
\newcommand{\SetStmt}{{\upshape\textsc{Set-Stmt}}}
\newcommand{\ManyOne}{{\upshape\textsc{Many-One}}}
\newcommand{\ManyMany}{{\upshape\textsc{Many-Many}}}

\newcommand{\MatA}{\mathbb{M}}

\newcommand{\SetSetCRBiv}{\rhd^{\mathsf{biv}}}
\newcommand{\SetFmlaCRBiv}{\vdash^{\mathsf{biv}}}

\newcommand{\SetSetCR}{\rhd}
\newcommand{\SetFmlaCR}{\vdash}
\newcommand{\SetFmlaComp}[1]{\vdash_{#1}}

\newcommand{\FmA}{\varphi}
\newcommand{\FmB}{\psi}
\newcommand{\FmC}{\gamma}
\newcommand{\FmD}{\delta}

\newcommand{\ValA}{x}
\newcommand{\ValB}{y}
\newcommand{\ValC}{z}

\newcommand{\FmSetA}{\Phi}
\newcommand{\FmSetB}{\Psi}
\newcommand{\FmSetC}{\Gamma}
\newcommand{\FmSetD}{\Pi}
\newcommand{\FmSetE}{\Delta}

\newcommand{\LabSysNameA}{\mathsf{G}}
\newcommand{\LabSysNameTriv}{\mathsf{G}_{\mathsf{triv}}}

%\newcommand{\CtxLabAOne}{\Phi_{\tv}}
%\newcommand{\CtxLabAHalf}{\Phi_{\uv}}
%\newcommand{\CtxLabAZero}{\Phi_{\bv}}

\newcommand{\CtxLabAOne}{\Gamma}
\newcommand{\CtxLabAHalf}{\Psi}
\newcommand{\CtxLabAZero}{\Phi}

\newcommand{\LabelValA}{\nu}
\newcommand{\LabFmSetA}{X}
\newcommand{\LabFmSetB}{Y}
\newcommand{\LabFmSetC}{Z}

\newcommand{\SetFmlaHRule}[3]{
    \AXC{\ensuremath{#1}}
    \LL{\ensuremath{#3}}
    \UIC{\ensuremath{#2}}
    \DP
}
\newcommand{\SetFmlaHName}{\mathcal{H}}

\newcommand{\ThreeLabName}[1]{\ell.{#1}}
\newcommand{\ThreeLabStreamName}[1]{s\ell.{#1}}

\newcommand{\MCRule}[2]{\frac{#1}{#2}}
\newcommand{\MCRuleInv}[2]{\frac{#2}{#1}}
\newcommand{\PropA}{p}
\newcommand{\PropB}{q}
\newcommand{\PropC}{r}
\newcommand{\PropD}{s}

\newcommand{\AlgInterp}[2]{{#1}_{#2}}

\newcommand{\SymbDef}{:=}

\newcommand{\ThreeValuesSet}{V_3}

\newcommand{\ValuesSetA}{V}
\newcommand{\DesSetA}{D}

\newcommand{\GenSubs}[1]{S}

\newcommand{\TPart}{T}
\newcommand{\FPart}{F}

\newcommand{\ValuesSetComp}[2]{{#1}{\setminus}{#2}}

\newcommand{\AlgA}{\mathbf{A}}

\newcommand{\TODO}[1]{{\color{blue}{\texttt{\textbf{[TODO]}} #1}}}

\newcommand{\dv}{d}
\newcommand{\uva}{u_1}
\newcommand{\uvb}{u_2}

\newcommand{\Sep}{\mathrm{S}}
\newcommand{\SepB}{\mathrm{U}}

\newcommand{\LukRule}[2]{\RuleA_{#1}}

\newcommand{\ArbDisj}{\oplus}
\newcommand{\ArbImp}{\rightarrowtriangle}

\newcommand{\LangAlgA}{\mathbf{L}_{\Sigma}(P)}
\newcommand{\LangSetA}{L_{\Sigma}(P)}

\newcommand{\LangSetAp}{L_{\Sigma}(\{\PropA\})}

\newcommand{\SigmaArity}[2]{{#1}^{(#2)}}

\newcommand{\Separates}[2]{{#1}\,\#\,{#2}}

\newcommand{\DesSeps}[1]{\Omega_{#1}}
\newcommand{\NDesSeps}[1]{\mho_{#1}}

\newcommand{\Hom}{\mathsf{Hom}}
\newcommand{\End}{\mathsf{End}}

\newcommand{\ValuationA}{v}

\newcommand{\CalcA}{\mathsf{R}}

\newcommand{\RuleA}{\mathsf{r}}

\newcommand{\AnalyticSetA}{\Theta}

\newcommand{\NSetSetCR}[1]{\blacktriangleright_{#1}}
\newcommand{\NSetSetCRBiv}[1]{\blacktriangleright_{#1}^{\mathsf{biv}}}

\newcommand{\REV}[1]{{\color{blue}#1}}

\newcommand{\FmSetComp}[1]{{#1}^{\mathsf{c}}}

\newcommand{\SetCut}{\Pi}

\newcommand{\AnaSetSetCR}[2]{\SetSetCR_{#1}^{#2}}
\newcommand{\NAnaSetSetCR}[2]{\NSetSetCR{#1}^{#2}}

\newcommand{\Subf}[1]{\mathsf{subf}(#1)}
\newcommand{\SubfTheta}[2]{\mathsf{subf}^{#1}(#2)}
\newcommand{\Props}[1]{\mathsf{props}(#1)}

\newcommand{\PowerSet}[1]{\mathcal{P}(#1)}

\newcommand{\TreeA}{\mathsf{t}}
\newcommand{\NodeA}{\mathsf{n}}

\newcommand{\Star}{\star}

\newcommand{\DNode}[2]{\ensuremath{{\OtherIfEmpty{#1}{#2}} ; {\OtherIfEmpty{#2}{#1}}}}

\newcommand{\SetFmlaRuleName}{r}
\newcommand{\SetFmlaCalculusName}{R}

\newcommand{\FmlasTree}[1]{\mathsf{fmlas}(#1)}

\newcommand{\NodeLabel}[2]{\mathsf{lab}^{#1}(#2)}
\newcommand{\ConA}{\textup{\copyright}}
%Giuseppe

\tikzset{
	treenode/.style = {align=center, inner sep=0pt, text centered},
	Ske/.style = {treenode, ellipse, double, draw=black,
		minimum width=6pt, thick},% arbre rouge noir, noeud noir
	PIA/.style = {treenode, ellipse, black, draw=black,
		minimum width=6pt},% arbre rouge noir, noeud rouge
	Crit/.style = {treenode, rectangle, draw=black,
		minimum width=0.5em, minimum height=0.5em}% arbre rouge noir, nil
}

\newcommand{\fns}{\footnotesize}

\def\fCenter{{\mbox{$\ \vdash\ $}}}
\def\ffCenter{{\mbox{$\overline{\vdash}$}}}
\def\fcenter{{\mbox{\ }}}


\newcommand{\mc}{\multicolumn}

%Multiplicative Operational connectives
\newcommand{\mtop}{1}
\newcommand{\mbot}{0}
\newcommand{\mand}{\otimes}
\newcommand{\mdlarr}{\varobslash}
\newcommand{\mdrarr}{\varoslash}
\newcommand{\mor}{\oplus}
\newcommand{\mrarr}{\,\,\backslash\,\,}
\newcommand{\mlarr}{\,\,\slash\,\,}
%
%Multiplicative Structural connectives
\newcommand{\MTOP}{\hat{1}}
\newcommand{\MBOT}{\check{0}}
\newcommand{\MAND}{\,\hat{\otimes}\,}
\newcommand{\MRARR}{\,\,\check{\backslash}\,\,}
\newcommand{\MLARR}{\,\check{\slash}\,}
\newcommand{\MOR}{\,\check{\oplus}\,}
\newcommand{\MDLARR}{\,\hat{\varobslash}\,}
\newcommand{\MDRARR}{\,\hat{\varoslash}\,}

%Distributive Lattice
%Operational Connectives
\newcommand{\aneg}{\ensuremath{\neg}\xspace}
\newcommand{\aatop}{\ensuremath{\top}\xspace}
\newcommand{\abot}{\ensuremath{\bot}\xspace}
\newcommand{\aand}{\ensuremath{\wedge}\xspace}
\newcommand{\aor}{\ensuremath{\vee}\xspace}
\newcommand{\ararr}{\ensuremath{\rightarrow}\xspace}
\newcommand{\alarr}{\ensuremath{\leftarrow}\xspace}
\newcommand{\alrarr}{\ensuremath{\leftrightarrow}\xspace}
\newcommand{\adrarr}{\ensuremath{\,{>\mkern-7mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\,}\xspace}
\newcommand{\adlarr}{\ensuremath{\rotatebox[origin=c]{180}{$\,>\mkern-8mu\raisebox{-0.065ex}{\aol}\,$}}\xspace}
%
%Structural Connectives
\newcommand{\ANEG}{\ensuremath{\:\tilde{\neg}}\xspace}
\newcommand{\ATOP}{\hat{\top}}
\newcommand{\ABOT}{\ensuremath{\check{\bot}}\xspace}
\newcommand{\AAND}{\ensuremath{\:\hat{\wedge}\:}\xspace}
\newcommand{\AOR}{\ensuremath{\:\check{\vee}\:}\xspace}
\newcommand{\ARARR}{\ensuremath{\:\check{\rightarrow}\:}\xspace}
\newcommand{\ALARR}{\ensuremath{\:\check{\leftarrow}\:}\xspace}
\newcommand{\ADRARR}{\ensuremath{\hat{{\:{>\mkern-7mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\:}}}\xspace}
\newcommand{\ADLARR}{\ensuremath{\:\hat{\rotatebox[origin=c]{180}{$\,>\mkern-8mu\raisebox{-0.065ex}{\aol}\,$}}\:}\xspace}

%Unary Modalities
%Operational connectives
\newcommand{\wbox}{\ensuremath{\Box}\xspace}
\newcommand{\wdia}{\ensuremath{\Diamond}\xspace}
\newcommand{\bbox}{\ensuremath{\blacksquare}\xspace}
\newcommand{\bdia}{\ensuremath{\Diamondblack}\xspace}
\newcommand{\bcirc}{\ensuremath{{\bullet}}\xspace}
\newcommand{\bboxdot}{\ensuremath{\boxdot}\xspace}
\newcommand{\bdialoz}{\ensuremath{\blacklozenge}\xspace}
%Structural connectives
\newcommand{\WBOX}{\ensuremath{\check{\Box}}\xspace}
\newcommand{\WDIA}{\ensuremath{\hat{\Diamond}}\xspace}
\newcommand{\BBOX}{\ensuremath{\check{\blacksquare}}\xspace}
\newcommand{\BDIA}{\ensuremath{\hat{\Diamondblack}}\xspace}
\newcommand{\WCIR}{\ensuremath{\tilde{{\circ}}}\xspace}
\newcommand{\BCIR}{\ensuremath{\tilde{{\bullet}}}\xspace}

\newcommand{\ders}{\vdash}
\newcommand{\derm} {\vartriangleright}
\newcommand{\Mt}{\mathbb{M}}
\newcommand{\tv}{\ensuremath{\mathbf 1}}
\newcommand{\tvb}{\ensuremath{\mathbf{\textcolor{blue}{1}}}}
%\newcommand{\uv}{\ensuremath{\mathbf{\nicefrac{1}{2}}}}

%UMBERTO:
\newcommand{\OLcon}{\ensuremath{\land_{\OL}}}
\newcommand{\OLdis}{\ensuremath{\lor_{\OL}}}
\newcommand{\OLimp}{\ensuremath{\to_{\OL}}}
\newcommand{\OLneg}{\ensuremath{\nnot_{\OL}}}

\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\alg}[1]{\mathbf{#1}}                  % algebras
\newcommand{\Al}[1][A]{\ensuremath{\mathbf{#1}} }
%\newcommand{\nnot}{\mathop{\sim}}                  % not
\newcommand{\nnot}{\mathop{\neg}}                  % not
\let\imp\Rightarrow                                % implies
\usepackage{amsmath, hyperref}
\newcommand{\pr}{\, \mathop{\preceq} \,}                 
 \newcommand{\eq}{\mathbin\equiv}
\def\zseq#1{\lseq #1 \rseq}                        % sequence
\def\zseq#1{\lseq #1 \rseq}                        % sequence
\let \lseq \langle                                 % left angle bracket
\let \rseq \rangle                                 % right angle bracket
\def\zset#1{\{ #1 \}}                              % set



\newcommand{\uv}{\ensuremath{\nicefrac{\mathbf{1}}{\mathbf{2}}}}
%\newcommand{\uv}{\ensuremath{\mathbf \top}}
\newcommand{\envert}[1]{\left\lvert#1\right\rvert}
\let\abs=\envert

\newcommand{\uvg}{\ensuremath{\mathbf{\textcolor{green}{\nicefrac{1}{2}}}}}
\newcommand{\bv}{\ensuremath{\mathbf{0}}}
\newcommand{\bvr}{\ensuremath{\mathbf{\textcolor{red}{0}}}}
 
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\newcommand{\smName}[1]{mc.{#1}}
\newcommand{\smcName}[1]{smc.{#1}}
 
 \newcommand{\sequent}{\Rightarrow{}}
 \newcommand{\half}{\frac{1}{2}}
%eheh, estamos na mesma linha! mas já vi que fizeste melhor! podes apagar a bagunça que fiz para aqui!

%Lattice cap
%Operational Connectives
\newcommand{\dneg}{\ensuremath{{\sim}}\xspace}
\newcommand{\rdneg}{\ensuremath{\neg}\xspace}
\newcommand{\dtop}{\ensuremath{1_\cap}\xspace}
\newcommand{\dbot}{\ensuremath{0_\cup}\xspace}
\newcommand{\dand}{\ensuremath{\cap}\xspace}
\newcommand{\dor}{\ensuremath{\cup}\xspace}
\newcommand{\drarr}{\ensuremath{>}\xspace}
\newcommand{\dcrarr}{\ensuremath{\,{>\mkern-7mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\,}\xspace}
%Structural Connectives
\newcommand{\DNEG}{\ensuremath{*}\xspace}
\newcommand{\ADNEG}{\ensuremath{\circledast}\xspace}
\newcommand{\DTOP}{\ensuremath{\hat{1_\cap}}\xspace}
\newcommand{\DBOT}{\ensuremath{\check{0_\cup}}\xspace}
\newcommand{\DAND}{\ensuremath{\:\hat{\cap}\:}\xspace}
\newcommand{\DOR}{\ensuremath{\:\check{\cup}\:}\xspace}
\newcommand{\DRARR}{\ensuremath{\:\check{>}\:}\xspace}
\newcommand{\DCRARR}{\ensuremath{\hat{{\:{>\mkern-7mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\:}}}\xspace}

%Lattice cup
%Operational Connectives
\newcommand{\utop}{\ensuremath{1}\xspace}
\newcommand{\ubot}{\ensuremath{0}\xspace}
\newcommand{\uand}{\sqcap}
\newcommand{\uor}{\sqcup}
\newcommand{\urarr}{\ensuremath{>}\xspace}
\newcommand{\ucrarr}{\ensuremath{\,{>\mkern-7mu\raisebox{-0.065ex}{\rule[0.5865ex]{1.38ex}{0.1ex}}}\,}\xspace}
%Structural Connectives
\newcommand{\UTOP}{\ensuremath{\hat{1}}\xspace}
\newcommand{\UBOT}{\ensuremath{\check{0}}\xspace}
\newcommand{\UAND}{\ensuremath{\:\hat{\sqcap}\:}\xspace}
\newcommand{\UOR}{\ensuremath{\:\check{\sqcup}\:}\xspace}
\newcommand{\URARR}{\ensuremath{\:\check{\sqsupset}\:}\xspace}
\newcommand{\UCRARR}{\ensuremath{\:\hat{\sqsubset}\:}\xspace}

%Sequents
\newcommand{\Sneg}{\ensuremath{{\sim}}\xspace}
\newcommand{\Rarr}{\ensuremath{\Rightarrow}\xspace}
\newcommand{\Srarr}{\ensuremath{\Rightarrow}\xspace}
\newcommand{\Sor}{\ensuremath{\parr}\xspace}
\newcommand{\Sand}{\ensuremath{\with}\xspace}
\newcommand{\BSor}{\ensuremath{\bigparr}\xspace}
\newcommand{\BSand}{\ensuremath{\bigwith}\xspace}
\newcommand{\D}{\ensuremath{\mathrm{D}}\xspace}
\newcommand{\U}{\ensuremath{\mathrm{U}}\xspace}

\newcommand{\SAND}{\ensuremath{\bigwith}\xspace}
\newcommand{\SOR}{\ensuremath{\bigparr}\xspace}


%ABrackets
%Angular brackets 
\newcommand{\lb}{\langle}
\newcommand{\rb}{\rangle}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}
            
%Translation brackets
\newcommand{\lf}{\lfloor}
\newcommand{\rf}{\rfloor}
\newcommand{\lc}{\lceil}
\newcommand{\rc}{\rceil}

\newcommand{\e}{\emptyset}


==> packages.tex <==
\usepackage{a4}
\usepackage[english]{babel}
\usepackage[dvipsnames,usenames]{color}

%\usepackage{authblk}

%\input{iscmac}
\usepackage{bbm}

\usepackage{verbatim,graphics,indentfirst} 
%\usepackage[mathscr]{euscript}
\usepackage{url}
\usepackage{stmaryrd}
\usepackage[nosumlimits]{amsmath}
%\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{amsthm}
\usepackage{float}
\usepackage{booktabs}

%\usepackage{mathtools}

\usepackage{latexsym}
\usepackage{enumerate}
\usepackage{graphicx}
%\usepackage{color}
\usepackage[T1]{fontenc}
%\usepackage[latin1]{inputenc}
\usepackage{lmodern}

\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{amsfonts}
\usepackage{nicefrac}
\usepackage{array}
\usepackage{appendix}

\usepackage{tikz}
\usepackage{tikz-qtree}
\usepackage[]{forest}

%Giuseppe packages
\usepackage{xspace}
\usepackage{marginnote}
\usepackage{bussproof}
\usepackage{cmll}

\usepackage{proof}

\usepackage{pdflscape}
%\usepackage{lscape}

\usepackage{tikz}

\usepackage{mathdots}

